ARC-GEN: A Mimetic Procedural Benchmark Generator for the Abstraction and Reasoning Corpus

The Abstraction and Reasoning Corpus remains one of the most compelling and challenging benchmarks for tracking progress toward achieving Artificial General Intelligence. In contrast to other evaluation datasets designed to assess an agent's task-specific skills or accumulated knowledge, the ARC-AGI suite is specifically targeted at measuring skill acquisition efficiency, a trait that has (so far) been lacking in even the most sophisticated machine learning systems. For algorithms that require extensive intra-task exemplars, a significant constraint imposed by ARC-AGI is the modest cardinality of its demonstration set, comprising a small number of $\langle$ input, output $\rangle$ grids per task specifying the corresponding transformation. To embellish the space of viable sample pairs, this paper introduces ARC-GEN, an open-source procedural generator aimed at extending the original ARC-AGI training dataset as faithfully as possible. Unlike prior efforts, our generator is both exhaustive (covering all four-hundred tasks) and mimetic (more closely honoring the distributional properties and characteristics embodied in the initial ARC-AGI-1 release). We also discuss the use of this generator in establishing a static benchmark suite to verify the correctness of programs submitted to the 2025 Google Code Golf Championship.

==> task007_code_compressed.tex <==
\textcolor{violet}{def} \textcolor{Orange}{p}(\textcolor{blue}{g}):
 \textcolor{blue}{a},\textcolor{blue}{b}=\textcolor{Maroon}{"eJyLjjb"},\textcolor{Maroon}{"GSsTrRSDwd"}
 \textcolor{blue}{c},\textcolor{blue}{d}=\textcolor{Maroon}{"yAfiadj"},\textcolor{Maroon}{"ORTpj4WA"}
 \textcolor{blue}{t}=[\textcolor{Maroon}{"SMdEx1I"},\textcolor{Maroon}{"SsdAx1o"},\textcolor{Maroon}{"RsdAx1o"}]
 \textcolor{blue}{u},\textcolor{blue}{v}=[\textcolor{Maroon}{"E"},\textcolor{Maroon}{"C"},\textcolor{Maroon}{"C"}],[\textcolor{Maroon}{"C"},\textcolor{Maroon}{"D"},\textcolor{Maroon}{"D"}]
 \textcolor{blue}{w}=[\textcolor{Maroon}{"EMyF6M="},\textcolor{Maroon}{"Fi2GAM="},\textcolor{Maroon}{"GBIGCU="}]
 \textcolor{blue}{i}=(\textcolor{darkgray}{1}-\textcolor{blue}{g}[\textcolor{darkgray}{4}][\textcolor{darkgray}{4}])*(\textcolor{darkgray}{1} \textcolor{violet}{if} \textcolor{blue}{g}[\textcolor{darkgray}{0}][\textcolor{darkgray}{0}] \textcolor{violet}{else} \textcolor{darkgray}{2})
 \textcolor{blue}{s}=\textcolor{blue}{a}+\textcolor{blue}{t}[\textcolor{blue}{i}]+\textcolor{blue}{b}+\textcolor{blue}{u}[\textcolor{blue}{i}]+\textcolor{blue}{c}+\textcolor{blue}{v}[\textcolor{blue}{i}]+\textcolor{blue}{d}+\textcolor{blue}{w}[\textcolor{blue}{i}]
 \textcolor{blue}{e}=\textcolor{ForestGreen}{base64}.\textcolor{Orange}{b64decode}(\textcolor{blue}{s}.\textcolor{Orange}{encode}())
 \textcolor{blue}{d}=\textcolor{ForestGreen}{zlib}.\textcolor{Orange}{decompress}(\textcolor{blue}{e}).\textcolor{Orange}{decode}()
 \textcolor{violet}{return} \textcolor{ForestGreen}{ast}.\textcolor{Orange}{literal_eval}(\textcolor{blue}{d})

==> task007_code_minimal.tex <==
\textcolor{violet}{def} \textcolor{Orange}{p}(\textcolor{blue}{g}):
 \textcolor{blue}{d},\textcolor{blue}{s}=[\textcolor{darkgray}{0}]*\textcolor{darkgray}{3},\textcolor{ForestGreen}{range}(\textcolor{ForestGreen}{len}(\textcolor{blue}{g}))
 \textcolor{violet}{for} _ \textcolor{violet}{in} \textcolor{blue}{d}:
  \textcolor{violet}{for} \textcolor{blue}{r} \textcolor{violet}{in} \textcolor{blue}{s}:
   \textcolor{violet}{for} \textcolor{blue}{c} \textcolor{violet}{in} \textcolor{blue}{s}:
    \textcolor{violet}{if} \textcolor{blue}{v}:=\textcolor{blue}{g}[\textcolor{blue}{r}][\textcolor{blue}{c}]:
     \textcolor{blue}{d}[(\textcolor{blue}{r}+\textcolor{blue}{c})\%\textcolor{darkgray}{3}]=\textcolor{blue}{v}
    \textcolor{blue}{g}[\textcolor{blue}{r}][\textcolor{blue}{c}]=\textcolor{blue}{d}[(\textcolor{blue}{r}+\textcolor{blue}{c})\%\textcolor{darkgray}{3}]
 \textcolor{violet}{return} \textcolor{blue}{g}

==> task032_code_compressed.tex <==
\textcolor{violet}{def} \textcolor{Orange}{p}(\textcolor{blue}{g}):
 \textcolor{blue}{n}=[\textcolor{darkgray}{4001469}, \textcolor{darkgray}{30000301063012},
    \textcolor{darkgray}{400000407800407809}]
 \textcolor{blue}{o},\textcolor{blue}{a},\textcolor{blue}{v}=[],[],\textcolor{blue}{n}[\textcolor{ForestGreen}{len}(\textcolor{blue}{g})-\textcolor{darkgray}{4}]
 \textcolor{violet}{for} \textcolor{blue}{r} \textcolor{violet}{in} \textcolor{blue}{g}:
  \textcolor{violet}{for} _ \textcolor{violet}{in} \textcolor{blue}{r}:
   \textcolor{blue}{a},\textcolor{blue}{v}=[\textcolor{blue}{v}\%\textcolor{darkgray}{10}]+\textcolor{blue}{a},\textcolor{blue}{v}//\textcolor{darkgray}{10}
  \textcolor{blue}{o},\textcolor{blue}{a}=[\textcolor{blue}{a}]+\textcolor{blue}{o},[]
 \textcolor{violet}{return} \textcolor{blue}{o}

==> task032_code_minimal.tex <==
\textcolor{violet}{def} \textcolor{Orange}{p}(\textcolor{blue}{g}):
 \textcolor{blue}{h},\textcolor{blue}{w}=\textcolor{ForestGreen}{len}(\textcolor{blue}{g}),\textcolor{ForestGreen}{len}(\textcolor{blue}{g}[\textcolor{darkgray}{0}])
 \textcolor{violet}{for} \textcolor{blue}{c} \textcolor{violet}{in} \textcolor{ForestGreen}{range}(\textcolor{blue}{w}):
  \textcolor{blue}{o}=\textcolor{blue}{h}-\textcolor{darkgray}{1}
  \textcolor{violet}{for} \textcolor{blue}{r} \textcolor{violet}{in} \textcolor{ForestGreen}{range}(\textcolor{blue}{o},\textcolor{darkgray}{-1},\textcolor{darkgray}{-1}):
   \textcolor{blue}{t},\textcolor{blue}{g}[\textcolor{blue}{r}][\textcolor{blue}{c}]=\textcolor{blue}{g}[\textcolor{blue}{r}][\textcolor{blue}{c}],\textcolor{darkgray}{0}
   \textcolor{violet}{if} \textcolor{blue}{t}:\textcolor{blue}{g}[\textcolor{blue}{o}][\textcolor{blue}{c}],\textcolor{blue}{o}=\textcolor{blue}{t},\textcolor{blue}{o}-\textcolor{darkgray}{1}
 \textcolor{violet}{return} \textcolor{blue}{g}

==> task125_generator.tex <==
\textcolor{violet}{def} \textcolor{Orange}{generate}(\textcolor{blue}{rows}=\textcolor{darkgray}{None}, \textcolor{blue}{cols}=\textcolor{darkgray}{None}, \textcolor{blue}{widths}=\textcolor{darkgray}{None}, \textcolor{blue}{heights}=\textcolor{darkgray}{None}, \textcolor{blue}{colors}=\textcolor{darkgray}{None},
             \textcolor{blue}{boxes}=\textcolor{darkgray}{3}, \textcolor{blue}{size}=\textcolor{darkgray}{15}):
 {\it\texttt{\textcolor{gray}{#### PARAMETERIZATION ####}}}
 \textcolor{violet}{if} \textcolor{blue}{rows} \textcolor{violet}{is} \textcolor{darkgray}{None}:
  \textcolor{violet}{while} \textcolor{darkgray}{True}:  {\it\texttt{\textcolor{gray}{# rows, cols = box coordinates ; widths, heights = box dimensions}}}
   \textcolor{blue}{widths}, \textcolor{blue}{heights} = \textcolor{ForestGreen}{common}.\textcolor{Orange}{randints}(\textcolor{darkgray}{2}, \textcolor{darkgray}{7}, \textcolor{blue}{boxes}), \textcolor{ForestGreen}{common}.\textcolor{Orange}{randints}(\textcolor{darkgray}{2}, \textcolor{darkgray}{7}, \textcolor{blue}{boxes})
   \textcolor{blue}{rows} = [\textcolor{ForestGreen}{common}.\textcolor{Orange}{randint}(\textcolor{darkgray}{1}, \textcolor{blue}{size} - \textcolor{blue}{height} - \textcolor{darkgray}{1}) \textcolor{violet}{for} \textcolor{blue}{height} \textcolor{violet}{in} \textcolor{blue}{heights}]
   \textcolor{blue}{cols} = [\textcolor{ForestGreen}{common}.\textcolor{Orange}{randint}(\textcolor{darkgray}{1}, \textcolor{blue}{size} - \textcolor{blue}{width} - \textcolor{darkgray}{1}) \textcolor{violet}{for} \textcolor{blue}{width} \textcolor{violet}{in} \textcolor{blue}{widths}]
   \textcolor{violet}{if} \textcolor{ForestGreen}{common}.\textcolor{Orange}{overlaps}(\textcolor{blue}{rows}, \textcolor{blue}{cols}, \textcolor{blue}{widths}, \textcolor{blue}{heights}, \textcolor{darkgray}{2}): \textcolor{violet}{continue}
   \textcolor{blue}{colors} = [\textcolor{ForestGreen}{common}.\textcolor{Orange}{pink}()] * \textcolor{blue}{boxes}
   \textcolor{blue}{newrows}, \textcolor{blue}{newcols}, \textcolor{blue}{newwidths}, \textcolor{blue}{newheights} = [], [], [], []
   \textcolor{violet}{for} \textcolor{blue}{row}, \textcolor{blue}{col}, \textcolor{blue}{width}, \textcolor{blue}{height} \textcolor{violet}{in}\ \textcolor{ForestGreen}{zip}(\textcolor{blue}{rows}, \textcolor{blue}{cols}, \textcolor{blue}{widths}, \textcolor{blue}{heights}):
    \textcolor{blue}{w}, \textcolor{blue}{t} = \textcolor{ForestGreen}{common}.\textcolor{Orange}{randint}(\textcolor{darkgray}{0}, \textcolor{blue}{width} - \textcolor{darkgray}{2}), \textcolor{ForestGreen}{common}.\textcolor{Orange}{randint}(\textcolor{darkgray}{0}, \textcolor{blue}{height} - \textcolor{darkgray}{2})
    \textcolor{violet}{if} \textcolor{violet}{not} \textcolor{blue}{w} \textcolor{violet}{or} \textcolor{violet}{not} \textcolor{blue}{t}: \textcolor{violet}{continue}
    \textcolor{blue}{r} = \textcolor{blue}{row} + \textcolor{ForestGreen}{common}.\textcolor{Orange}{randint}(\textcolor{darkgray}{1}, \textcolor{blue}{height} - \textcolor{blue}{t} - \textcolor{darkgray}{1})
    \textcolor{blue}{c} = \textcolor{blue}{col} + \textcolor{ForestGreen}{common}.\textcolor{Orange}{randint}(\textcolor{darkgray}{1}, \textcolor{blue}{width} - \textcolor{blue}{w} - \textcolor{darkgray}{1})
    \textcolor{blue}{newrows}, \textcolor{blue}{newcols} = \textcolor{blue}{newrows} + [\textcolor{blue}{r}], \textcolor{blue}{newcols} + [\textcolor{blue}{c}]
    \textcolor{blue}{newwidths}, \textcolor{blue}{newheights} = \textcolor{blue}{newwidths} + [\textcolor{blue}{w}], \textcolor{blue}{newheights} + [\textcolor{blue}{t}]
   \textcolor{violet}{if} \textcolor{ForestGreen}{sum}(\textcolor{blue}{w} * \textcolor{blue}{t} \textcolor{violet}{for} \textcolor{blue}{w}, \textcolor{blue}{t} \textcolor{violet}{in} \textcolor{ForestGreen}{zip}(\textcolor{blue}{newwidths}, \textcolor{blue}{newheights})) < \textcolor{darkgray}{2} * \textcolor{blue}{boxes}: \textcolor{violet}{continue}
   \textcolor{blue}{rows}, \textcolor{blue}{cols} = \textcolor{blue}{rows} + \textcolor{blue}{newrows}, \textcolor{blue}{cols} + \textcolor{blue}{newcols}
   \textcolor{blue}{widths}, \textcolor{blue}{heights} = \textcolor{blue}{widths} + \textcolor{blue}{newwidths}, \textcolor{blue}{heights} + \textcolor{blue}{newheights}
   \textcolor{blue}{colors}.\textcolor{Orange}{extend}([\textcolor{ForestGreen}{common}.\textcolor{Orange}{yellow}()] * \textcolor{ForestGreen}{len}(\textcolor{blue}{newrows}))
   \textcolor{violet}{break}

 {\it\texttt{\textcolor{gray}{#### GENERATION ####}}}
 \textcolor{blue}{grid}, \textcolor{blue}{output} = \textcolor{ForestGreen}{common}.\textcolor{Orange}{grids}(\textcolor{blue}{size}, \textcolor{blue}{size}, \textcolor{ForestGreen}{common}.\textcolor{Orange}{cyan}())
 \textcolor{violet}{for} \textcolor{blue}{row}, \textcolor{blue}{col}, \textcolor{blue}{width}, \textcolor{blue}{height}, \textcolor{blue}{color} \textcolor{violet}{in} \textcolor{ForestGreen}{zip}(\textcolor{blue}{rows}, \textcolor{blue}{cols}, \textcolor{blue}{widths}, \textcolor{blue}{heights}, \textcolor{blue}{colors}):
  \textcolor{violet}{for} \textcolor{blue}{r} \textcolor{violet}{in} \textcolor{ForestGreen}{range}(\textcolor{blue}{row} - \textcolor{darkgray}{1}, \textcolor{blue}{row} + \textcolor{blue}{height} + \textcolor{darkgray}{1}):
   \textcolor{violet}{for} \textcolor{blue}{c} \textcolor{violet}{in} \textcolor{ForestGreen}{range}(\textcolor{blue}{col} - \textcolor{darkgray}{1}, \textcolor{blue}{col} + \textcolor{blue}{width} + \textcolor{darkgray}{1}):
    \textcolor{violet}{if} \textcolor{blue}{color} == \textcolor{ForestGreen}{common}.\textcolor{Orange}{pink}(): \textcolor{blue}{output}[\textcolor{blue}{r}][\textcolor{blue}{c}] = \textcolor{ForestGreen}{common}.\textcolor{Orange}{green}()
    \textcolor{violet}{if} \textcolor{blue}{r} < \textcolor{blue}{row} \textcolor{violet}{or} \textcolor{blue}{r} >= \textcolor{blue}{row} + \textcolor{blue}{height} \textcolor{violet}{or} \textcolor{blue}{c} < \textcolor{blue}{col} \textcolor{violet}{or} \textcolor{blue}{c} >= \textcolor{blue}{col} + \textcolor{blue}{width}: \textcolor{violet}{continue}
    \textcolor{blue}{grid}[\textcolor{blue}{r}][\textcolor{blue}{c}] = \textcolor{blue}{color} \textcolor{violet}{if} \textcolor{blue}{color} == \textcolor{ForestGreen}{common}.\textcolor{Orange}{pink}() \textcolor{violet}{else} \textcolor{ForestGreen}{common}.\textcolor{Orange}{cyan}()
    \textcolor{blue}{output}[\textcolor{blue}{r}][\textcolor{blue}{c}] = \textcolor{blue}{color}
 \textcolor{violet}{return} \{\textcolor{Maroon}{"input"}: \textcolor{blue}{grid}, \textcolor{Maroon}{"output"}: \textcolor{blue}{output}\}

{\it\texttt{\textcolor{gray}{#### VALIDATION ####}}}
\textcolor{violet}{def} \textcolor{Orange}{validate}():
 \textcolor{blue}{train} = [\textcolor{Orange}{generate}(\textcolor{blue}{rows}=[\textcolor{darkgray}{2}, \textcolor{darkgray}{4}, \textcolor{darkgray}{10}, \textcolor{darkgray}{3}], \textcolor{blue}{cols}=[\textcolor{darkgray}{8}, \textcolor{darkgray}{3}, \textcolor{darkgray}{5}, \textcolor{darkgray}{9}], \textcolor{blue}{widths}=[\textcolor{darkgray}{4}, \textcolor{darkgray}{2}, \textcolor{darkgray}{4}, \textcolor{darkgray}{2}],
                   \textcolor{blue}{heights}=[\textcolor{darkgray}{5}, \textcolor{darkgray}{2}, \textcolor{darkgray}{4}, \textcolor{darkgray}{3}], \textcolor{blue}{colors}=[\textcolor{darkgray}{6}, \textcolor{darkgray}{6}, \textcolor{darkgray}{6}, \textcolor{darkgray}{4}]),
          \textcolor{Orange}{generate}(\textcolor{blue}{rows}=[\textcolor{darkgray}{1}, \textcolor{darkgray}{3}, \textcolor{darkgray}{8}, \textcolor{darkgray}{4}, \textcolor{darkgray}{9}], \textcolor{blue}{cols}=[\textcolor{darkgray}{8}, \textcolor{darkgray}{2}, \textcolor{darkgray}{8}, \textcolor{darkgray}{3}, \textcolor{darkgray}{9}],
                   \textcolor{blue}{widths}=[\textcolor{darkgray}{3}, \textcolor{darkgray}{4}, \textcolor{darkgray}{6}, \textcolor{darkgray}{1}, \textcolor{darkgray}{4}], \textcolor{blue}{heights}=[\textcolor{darkgray}{3}, \textcolor{darkgray}{4}, \textcolor{darkgray}{6}, \textcolor{darkgray}{2}, \textcolor{darkgray}{4}],
                   \textcolor{blue}{colors}=[\textcolor{darkgray}{6}, \textcolor{darkgray}{6}, \textcolor{darkgray}{6}, \textcolor{darkgray}{4}, \textcolor{darkgray}{4}])]
 \textcolor{blue}{test} = [\textcolor{Orange}{generate}(\textcolor{blue}{rows}=[\textcolor{darkgray}{2}, \textcolor{darkgray}{3}, \textcolor{darkgray}{11}, \textcolor{darkgray}{4}, \textcolor{darkgray}{4}, \textcolor{darkgray}{12}], \textcolor{blue}{cols}=[\textcolor{darkgray}{9}, \textcolor{darkgray}{2}, \textcolor{darkgray}{4}, \textcolor{darkgray}{10}, \textcolor{darkgray}{3}, \textcolor{darkgray}{6}],
                  \textcolor{blue}{widths}=[\textcolor{darkgray}{3}, \textcolor{darkgray}{4}, \textcolor{darkgray}{7}, \textcolor{darkgray}{1}, \textcolor{darkgray}{2}, \textcolor{darkgray}{2}], \textcolor{blue}{heights}=[\textcolor{darkgray}{6}, \textcolor{darkgray}{4}, \textcolor{darkgray}{3}, \textcolor{darkgray}{3}, \textcolor{darkgray}{2}, \textcolor{darkgray}{1}],
                  \textcolor{blue}{colors}=[\textcolor{darkgray}{6}, \textcolor{darkgray}{6}, \textcolor{darkgray}{6}, \textcolor{darkgray}{4}, \textcolor{darkgray}{4}, \textcolor{darkgray}{4}])]
 \textcolor{violet}{return} \{\textcolor{Maroon}{"train"}: \textcolor{blue}{train}, \textcolor{Maroon}{"test"}: \textcolor{blue}{test}\}

==> task151_code_compressed.tex <==
\textcolor{violet}{def} \textcolor{Orange}{p}(\textcolor{blue}{g}):
 \textcolor{blue}{n}=[[(\textcolor{darkgray}{0},\textcolor{darkgray}{0}),(\textcolor{darkgray}{0},\textcolor{darkgray}{1}),(\textcolor{darkgray}{0},\textcolor{darkgray}{2}),(\textcolor{darkgray}{1},\textcolor{darkgray}{0}),
     (\textcolor{darkgray}{1},\textcolor{darkgray}{2}),(\textcolor{darkgray}{2},\textcolor{darkgray}{0}),(\textcolor{darkgray}{2},\textcolor{darkgray}{1}),(\textcolor{darkgray}{2},\textcolor{darkgray}{2})],
    [(\textcolor{darkgray}{1},\textcolor{darkgray}{1}),(\textcolor{darkgray}{1},\textcolor{darkgray}{2}),(\textcolor{darkgray}{1},\textcolor{darkgray}{3}),(\textcolor{darkgray}{2},\textcolor{darkgray}{1}),
     (\textcolor{darkgray}{2},\textcolor{darkgray}{3}),(\textcolor{darkgray}{3},\textcolor{darkgray}{1}),(\textcolor{darkgray}{3},\textcolor{darkgray}{2}),(\textcolor{darkgray}{3},\textcolor{darkgray}{3})],
    [(\textcolor{darkgray}{3},\textcolor{darkgray}{3}),(\textcolor{darkgray}{3},\textcolor{darkgray}{4}),(\textcolor{darkgray}{3},\textcolor{darkgray}{5}),(\textcolor{darkgray}{4},\textcolor{darkgray}{3}),
     (\textcolor{darkgray}{4},\textcolor{darkgray}{5}),(\textcolor{darkgray}{5},\textcolor{darkgray}{3}),(\textcolor{darkgray}{5},\textcolor{darkgray}{4}),(\textcolor{darkgray}{5},\textcolor{darkgray}{5})]]
 \textcolor{violet}{for} \textcolor{blue}{r},\textcolor{blue}{c} \textcolor{violet}{in} \textcolor{blue}{n}[\textcolor{ForestGreen}{len}(\textcolor{blue}{g})//\textcolor{darkgray}{2}-\textcolor{darkgray}{2}]:
  \textcolor{blue}{g}[\textcolor{blue}{r}][\textcolor{blue}{c}]=\textcolor{darkgray}{4}
 \textcolor{violet}{return} \textcolor{blue}{g}

==> task151_code_minimal.tex <==
\textcolor{violet}{def} \textcolor{Orange}{p}(\textcolor{blue}{g}):
 \textcolor{blue}{s},\textcolor{blue}{x},\textcolor{blue}{y}=\textcolor{ForestGreen}{range}(\textcolor{darkgray}{1},\textcolor{ForestGreen}{len}(\textcolor{blue}{g})-\textcolor{darkgray}{1}),\textcolor{darkgray}{0},\textcolor{darkgray}{0}
 \textcolor{violet}{for} \textcolor{blue}{r} \textcolor{violet}{in} \textcolor{blue}{s}:
  \textcolor{violet}{for} \textcolor{blue}{c} \textcolor{violet}{in} \textcolor{blue}{s}:
   \textcolor{blue}{m}=\textcolor{blue}{g}[\textcolor{blue}{r}][\textcolor{blue}{c}-\textcolor{darkgray}{1}]*\textcolor{blue}{g}[\textcolor{blue}{r}][\textcolor{blue}{c}+\textcolor{darkgray}{1}]
   \textcolor{violet}{if} \textcolor{blue}{m}*\textcolor{blue}{g}[\textcolor{blue}{r}-\textcolor{darkgray}{1}][\textcolor{blue}{c}]*\textcolor{blue}{g}[\textcolor{blue}{r}+\textcolor{darkgray}{1}][\textcolor{blue}{c}]:
    \textcolor{blue}{x},\textcolor{blue}{y}=\textcolor{blue}{r},\textcolor{blue}{c}
 \textcolor{violet}{for} \textcolor{blue}{i} \textcolor{violet}{in} \textcolor{ForestGreen}{range}(\textcolor{darkgray}{9}):
  \textcolor{violet}{if} \textcolor{blue}{i}!=\textcolor{darkgray}{4}:\textcolor{blue}{g}[\textcolor{blue}{x}+\textcolor{blue}{i}//\textcolor{darkgray}{3}-\textcolor{darkgray}{1}][\textcolor{blue}{y}+\textcolor{blue}{i}\%\textcolor{darkgray}{3}-\textcolor{darkgray}{1}]=\textcolor{darkgray}{4}
 \textcolor{violet}{return} \textcolor{blue}{g}
